Boltzmann sampling for an XY model using a non-degenerate optical parametric oscillator network

We present an experimental scheme of implementing multiple spins in a classical XY model using a non-degenerate optical parametric oscillator (NOPO) network. We built an NOPO network to simulate a one-dimensional XY Hamiltonian with 5000 spins and externally controllable effective temperatures. The XY spin variables in our scheme are mapped onto the phases of multiple NOPO pulses in a single ring cavity and interactions between XY spins are implemented by mutual injections between NOPOs. We show the steady-state distribution of optical phases of such NOPO pulses is equivalent to the Boltzmann distribution of the corresponding XY model. Estimated effective temperatures converged to the setting values, and the estimated temperatures and the mean energy exhibited good agreement with the numerical simulations of the Langevin dynamics of NOPO phases.

==> commands.tex <==
\newcommand{\nn}{\notag \\}
\newcommand{\noin}{\\ \noindent}
\newcommand{\intf}{\int^{\infty}_{-\infty}}
\newcommand{\refs}[1]{(\ref{#1})}
\newcommand{\eq}[1]{\begin{equation} #1 \end{equation}}
\newcommand{\al}[1]{\begin{align} #1 \end{align}}		
\newcommand{\ang}[1]{\left \langle #1 \right \rangle}	
\newcommand{\rct}[1]{\left [ #1 \right ]}	
\newcommand{\abs}[1]{\left | #1 \right |}	
\newcommand{\prn}[1]{\left ( #1 \right )}	
\newcommand{\clb}[1]{\left \{ #1 \right \}}
\newcommand{\ket}[1]{\left | #1 \right \rangle}	
\newcommand{\bra}[1]{\left \langle #1 \right |}
\newcommand{\fracp}[2]{\left ( \frac{#1}{#2} \right )}	
\newcommand{\eqsp}[1]{\begin{equation} \begin{split} #1 \end{split} \end{equation}}
\newcommand{\sbrm}[1]{_{\mathrm{#1}}}
\newcommand{\bfit}[1]{\mbox{\boldmath $#1$}}
\newcommand{\fig}[4]{\begin{figure}[H] \centering \includegraphics[width = #2 cm]{#1} \caption{#3} \label{#4} \end{figure} }
\newcommand{\tbl}[5]{\begin{table}[H] \caption{#1} \label{#2} \begin{center} \begin{tabular} {#3} \toprule #4  \midrule #5 \bottomrule \end{tabular} \end{center} \end{table}}
\newcommand{\tbln}[4]{\begin{table}[H] \caption{#1} \label{#2} \begin{center} \begin{tabular} {#3} \toprule #4 \bottomrule \end{tabular} \end{center} \end{table}}


\newcommand{\ox}{\otimes} 
\newcommand{\schrodinger}{$\mathrm{Schr\ddot{o}dinger}$}
\newcommand{\tr}{\mathrm{tr}} 
\newcommand{\dg}{^\dagger}

\newcommand{\ptd}[1]{\frac{\partial}{\partial #1}}
